Uneven gains in protein-RNA affinity and mutation-effect prediction

Accurate matched affinities determine mutation effects, but gains in aggregate affinity prediction may transfer unevenly to average effects, ordering and local accuracy. We evaluated eleven method families using method-specific matched populations. Controlled CoPRA reduced absolute-affinity mean absolute error from 1.2898 to 1.1431 pKd. Across 220 mutation pairs from 20 families, it generated stronger responses and improved mean-effect accuracy, with uncertain ranking gains and no decrease in mean centered local error. In an independent external test (24 quantitative pairs from three source-matched families), absolute and ordinary mutation-effect errors fell in all three families. Mean centered local error fell from 0.4198 to 0.3761 pKd, with improvements in two families and higher error in one. Error decomposition localized gains in landscape means. PRA-Pred feature tracing, fixed-weight M2-PRNet input controls and matched supervision interventions identified specific restrictions on mutation response. These results establish the need to evaluate average effects, ordering and quantitative local variation jointly.

==> table4.tex <==
\begin{table*}[!htbp]
\centering
\caption{\textbf{Modeling interventions and reference-anchored decoupling across matched cohorts.}}
\label{tab:rapd}
\begingroup\fontsize{8.5}{10.4}\selectfont\setlength{\tabcolsep}{2.5pt}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lrrrrr@{}}\toprule
\textbf{Model} & Abs. MAE & Ord. $\Delta$MAE & Local cMAE & Pos. Spearman & SD ratio\\\midrule
\multicolumn{6}{@{}l}{\textbf{A. Principal full cohort} (752 absolute units, 338 ordinary pairs, 220 local pairs, 20 local families)}\\[3pt]
Controlled CoPRA (reference) & $1.1431$ & $0.7917$ & $0.3991$ & $0.1886$ & $0.6422$\\[2pt]
Additive comparator & \shortstack[r]{$1.2898$\\[-1pt]{\scriptsize $[+0.0545,\,+0.2424]$}} & \shortstack[r]{$0.8629$\\[-1pt]{\scriptsize $[+0.0362,\,+0.1068]$}} & \shortstack[r]{$0.3749$\\[-1pt]{\scriptsize $[-0.0635,\,+0.0088]$}} & \shortstack[r]{$0.1481$\\[-1pt]{\scriptsize $[-0.1645,\,+0.0822]$}} & \shortstack[r]{$0.0709$\\[-1pt]{\scriptsize $[-0.9560,\,-0.2808]$}}\\[2pt]
Zero-change reference & --- & \shortstack[r]{$0.8816$\\[-1pt]{\scriptsize $[+0.0509,\,+0.1284]$}} & \shortstack[r]{$0.3787$\\[-1pt]{\scriptsize $[-0.0609,\,+0.0151]$}} & --- & \shortstack[r]{$0.0000$\\[-1pt]{\scriptsize $[-1.0322,\,-0.3417]$}}\\[2pt]
cMAE-selected readout\textsuperscript{a} & --- & \shortstack[r]{$0.8816$\\[-1pt]{\scriptsize $[+0.0509,\,+0.1284]$}} & \shortstack[r]{$0.3787$\\[-1pt]{\scriptsize $[-0.0609,\,+0.0151]$}} & --- & \shortstack[r]{$0.0000$\\[-1pt]{\scriptsize $[-1.0322,\,-0.3417]$}}\\[2pt]
Endpoint-sum potential & \shortstack[r]{$1.1464$\\[-1pt]{\scriptsize $[-0.0500,\,+0.0587]$}} & \shortstack[r]{$0.8107$\\[-1pt]{\scriptsize $[-0.0021,\,+0.0385]$}} & \shortstack[r]{$0.3727$\\[-1pt]{\scriptsize $[-0.0516,\,-0.0050]$}} & \shortstack[r]{$0.2052$\\[-1pt]{\scriptsize $[-0.0227,\,+0.0586]$}} & \shortstack[r]{$0.3389$\\[-1pt]{\scriptsize $[-0.4984,\,-0.1537]$}}\\[2pt]
Decoupled AA-only & $1.1431$\textsuperscript{\dag} & \shortstack[r]{$0.8192$\\[-1pt]{\scriptsize $[+0.0052,\,+0.0483]$}} & \shortstack[r]{$0.3749$\\[-1pt]{\scriptsize $[-0.0499,\,-0.0018]$}} & \shortstack[r]{$0.1919$\\[-1pt]{\scriptsize $[-0.0070,\,+0.0142]$}} & \shortstack[r]{$0.3214$\\[-1pt]{\scriptsize $[-0.5156,\,-0.1709]$}}\\[2pt]
Decoupled 3D-Ridge & $1.1431$\textsuperscript{\dag} & \shortstack[r]{$0.8071$\\[-1pt]{\scriptsize $[-0.0050,\,+0.0348]$}} & \shortstack[r]{$0.3731$\\[-1pt]{\scriptsize $[-0.0489,\,-0.0052]$}} & \shortstack[r]{$0.2689$\\[-1pt]{\scriptsize $[-0.0046,\,+0.1981]$}} & \shortstack[r]{$0.3516$\\[-1pt]{\scriptsize $[-0.4693,\,-0.1488]$}}\\[2pt]
\textbf{RAPD} & $1.1431$\textsuperscript{\dag} & \shortstack[r]{$0.7704$\\[-1pt]{\scriptsize $[-0.0418,\,+0.0005]$}} & \shortstack[r]{$0.3660$\\[-1pt]{\scriptsize $[-0.0569,\,-0.0120]$}} & \shortstack[r]{$0.3123$\\[-1pt]{\scriptsize $[+0.0109,\,+0.2596]$}} & \shortstack[r]{$0.4700$\\[-1pt]{\scriptsize $[-0.3052,\,-0.0534]$}}\\[2pt]
\midrule
\multicolumn{6}{@{}l}{\textbf{B. Principal subset without detected PRA310 overlap} (95 absolute units, 53 ordinary pairs, 35 local pairs)}\\[3pt]
Controlled CoPRA (matched subset) & $1.5154$ & $0.5741$ & $0.4176$ & $0.1553$ & $0.3487$\\[2pt]
Official Released CoPRA & \shortstack[r]{$1.6776$\\[-1pt]{\scriptsize $[-0.3334,\,+0.6904]$}} & \shortstack[r]{$0.6304$\\[-1pt]{\scriptsize $[+0.0144,\,+0.1010]$}} & \shortstack[r]{$0.4244$\\[-1pt]{\scriptsize $[-0.0112,\,+0.0358]$}} & \shortstack[r]{$-0.1065$\\[-1pt]{\scriptsize $[-0.8029,\,+0.3865]$}} & \shortstack[r]{$0.0016$\\[-1pt]{\scriptsize $[-0.3936,\,-0.3208]$}}\\[2pt]
\midrule
\multicolumn{6}{@{}l}{\textbf{C. Independent external test} (27 absolute units, 24 pairs, 3 source-matched families)}\\[3pt]
Controlled CoPRA & \shortstack[r]{$0.5282$\\[-1pt]{\scriptsize $[0.3770,\,0.8289]$}} & \shortstack[r]{$0.6995$\\[-1pt]{\scriptsize $[0.3982,\,1.0317]$}} & \shortstack[r]{$0.3761$\\[-1pt]{\scriptsize $[0.3357,\,0.3978]$}} & \shortstack[r]{$0.1454$\\[-1pt]{\scriptsize $[-0.2619,\,0.4095]$}} & \shortstack[r]{$0.3900$\\[-1pt]{\scriptsize $[0.3067,\,0.4692]$}}\\[2pt]
Official Released CoPRA & \shortstack[r]{$1.4606$\\[-1pt]{\scriptsize $[0.6353,\,1.8769]$}} & \shortstack[r]{$0.9320$\\[-1pt]{\scriptsize $[0.4945,\,1.3977]$}} & \shortstack[r]{$0.4241$\\[-1pt]{\scriptsize $[0.3704,\,0.4902]$}} & \shortstack[r]{$-0.2112$\\[-1pt]{\scriptsize $[-0.4857,\,0.1071]$}} & \shortstack[r]{$0.0149$\\[-1pt]{\scriptsize $[0.0070,\,0.0222]$}}\\[2pt]
Additive comparator & \shortstack[r]{$0.6932$\\[-1pt]{\scriptsize $[0.4483,\,0.9397]$}} & \shortstack[r]{$0.8845$\\[-1pt]{\scriptsize $[0.4866,\,1.2998]$}} & \shortstack[r]{$0.4198$\\[-1pt]{\scriptsize $[0.3553,\,0.4869]$}} & \shortstack[r]{$0.2208$\\[-1pt]{\scriptsize $[-0.2571,\,0.7024]$}} & \shortstack[r]{$0.0467$\\[-1pt]{\scriptsize $[0.0173,\,0.0786]$}}\\[2pt]
\shortstack[l]{Zero-change /\\cMAE-selected readout} & --- & \shortstack[r]{$0.9223$\\[-1pt]{\scriptsize $[0.4926,\,1.3803]$}} & \shortstack[r]{$0.4230$\\[-1pt]{\scriptsize $[0.3688,\,0.4892]$}} & --- & \shortstack[r]{$0.0000$\\[-1pt]{\scriptsize $[0.0000,\,0.0000]$}}\\[2pt]
Endpoint-sum potential & \shortstack[r]{$0.5849$\\[-1pt]{\scriptsize $[0.4029,\,0.8701]$}} & \shortstack[r]{$0.7860$\\[-1pt]{\scriptsize $[0.4369,\,1.1652]$}} & \shortstack[r]{$0.3935$\\[-1pt]{\scriptsize $[0.3642,\,0.4383]$}} & \shortstack[r]{$0.1811$\\[-1pt]{\scriptsize $[-0.1190,\,0.3905]$}} & \shortstack[r]{$0.2023$\\[-1pt]{\scriptsize $[0.1613,\,0.2429]$}}\\[2pt]
Decoupled AA-only & \shortstack[r]{$0.5282$\\[-1pt]{\scriptsize $[0.3770,\,0.8289]$}} & \shortstack[r]{$0.7994$\\[-1pt]{\scriptsize $[0.4347,\,1.2005]$}} & \shortstack[r]{$0.3959$\\[-1pt]{\scriptsize $[0.3732,\,0.4399]$}} & \shortstack[r]{$0.1403$\\[-1pt]{\scriptsize $[-0.2619,\,0.4095]$}} & \shortstack[r]{$0.1951$\\[-1pt]{\scriptsize $[0.1535,\,0.2344]$}}\\[2pt]
Decoupled 3D-Ridge & \shortstack[r]{$0.5282$\\[-1pt]{\scriptsize $[0.3770,\,0.8289]$}} & \shortstack[r]{$0.7895$\\[-1pt]{\scriptsize $[0.4270,\,1.2200]$}} & \shortstack[r]{$0.4073$\\[-1pt]{\scriptsize $[0.3775,\,0.4301]$}} & \shortstack[r]{$0.1560$\\[-1pt]{\scriptsize $[-0.4881,\,0.5810]$}} & \shortstack[r]{$0.2358$\\[-1pt]{\scriptsize $[0.1692,\,0.3203]$}}\\[2pt]
\textbf{RAPD} & \shortstack[r]{$0.5282$\\[-1pt]{\scriptsize $[0.3770,\,0.8289]$}} & \shortstack[r]{$0.7207$\\[-1pt]{\scriptsize $[0.4111,\,1.1416]$}} & \shortstack[r]{$0.4151$\\[-1pt]{\scriptsize $[0.4075,\,0.4241]$}} & \shortstack[r]{$0.0950$\\[-1pt]{\scriptsize $[-0.3929,\,0.3827]$}} & \shortstack[r]{$0.2677$\\[-1pt]{\scriptsize $[0.2231,\,0.3071]$}}\\[2pt]
\bottomrule\end{tabular*}\par\smallskip
\noindent\begin{minipage}{\textwidth}\raggedright
Brackets in panels A and B give paired 95\% family-bootstrap intervals for model minus matched Controlled CoPRA. Negative values indicate lower error for MAE metrics, and positive values indicate higher rank correlation or amplitude. Panel C gives equally weighted family means with observed minima and maxima in brackets. Dashes denote undefined or unavailable metrics. Errors are in pKd. \textsuperscript{a}All four readouts (hidden representation, contact, hybrid and amino-acid composition) selected zero response in each outer fold. \textsuperscript{\dag}Identical to the Controlled CoPRA absolute-affinity output by construction.
\end{minipage}\endgroup\end{table*}

